The Green Choice: Learning and Influencing Human Decisions on Shared Roads

Autonomous vehicles have the potential to increase the capacity of roads via platooning, even when human drivers and autonomous vehicles share roads. However, when users of a road network choose their routes selfishly, the resulting traffic configuration may be very inefficient. Because of this, we consider how to influence human decisions so as to decrease congestion on these roads. We consider a network of parallel roads with two modes of transportation: (i) human drivers who will choose the quickest route available to them, and (ii) ride hailing service which provides an array of autonomous vehicle ride options, each with different prices, to users. In this work, we seek to design these prices so that when autonomous service users choose from these options and human drivers selfishly choose their resulting routes, road usage is maximized and transit delay is minimized. To do so, we formalize a model of how autonomous service users make choices between routes with different price/delay values. Developing a preference-based algorithm to learn the preferences of the users, and using a vehicle flow model related to the Fundamental Diagram of Traffic, we formulate a planning optimization to maximize a social objective and demonstrate the benefit of the proposed routing and learning scheme.

==> experiments.tex <==
To validate our framework, we conducted simulations and user studies. We test three hypotheses that together suggest our framework successfully reduces traffic congestion through pricing, after it effectively learns the humans' choice models:\\
\textbf{H1}: Our active learning algorithm is able to learn the presented human choice model in a data-efficient way.\\
\textbf{H2}: Our traffic optimization reduces the latencies by creating altruistic behavior through pricing.\\
\textbf{H3}: When used by real humans, the overall framework works well and is advantageous over non-altruistic algorithms.

To test \textbf{H1}, we simulated $5$ autonomous service users who have different preferences, which are designed to be realistic, and used them for our simulations. We tested our data-efficient learning framework. We asked two sets of $60$ queries, each of which consisted of $4$ road options and a walking option, to the simulated users. The queries were generated actively in the first set and randomly in the second. After each query, we recorded the sample $(\bar{\boldsymbol{\omega}},\bar\zeta)$ which has the highest likelihood.

For \textbf{H3}, we recruited $21$ subjects ($9$ female, $12$ male) with an age range from 19 to 60. To increase the diversity among user preferences, the subjects are selected from a diverse set of locations: California / Georgia / Illinois, USA; Ankara / Denizli, Turkey; Singapore. \erdem{This sounds cool, but we may actually remove this. I ran a two-sample t-test on USA vs Turkey, and there were no significant differences...}

\ramtin{Let's start more high level instead of the details and numerical values of parameters. E.g., what is the evaluation plan? What is the procedure for the experiments?} In all of our experiments, we assumed there is only one alternative option for autonomous users, and it is walking to the destination. We set $c=6\times 10^{-5}$ USD/meter. We assumed the human-driven cars keep a $2$-second headway distance with the leading car, whereas autonomous cars keep $1$-second distance. We set the length of the cars as $5$ meters, and the minimum gap between two cars as $2$ meters.
\dorsa{I agree with Ramtin. First give a high level idea of what you're experimenting and again what the goal was. The specific paragraph above should go under a subparagraph called something like the details of the experiment.}

